A Recipe For Arbitrary Text Style Transfer with Large Language Models

In this paper, we leverage large language models (LMs) to perform zero-shot text style transfer. We present a prompting method that we call augmented zero-shot learning, which frames style transfer as a sentence rewriting task and requires only a natural language instruction, without model fine-tuning or exemplars in the target style. Augmented zero-shot learning is simple and demonstrates promising results not just on standard style transfer tasks such as sentiment, but also on arbitrary transformations such as "make this melodramatic" or "insert a metaphor."

==> tables/fs_prompts.tex <==
\newcommand{\inputsent}[1]{\textcolor{teal}{\{#1\}}}
\newcommand{\rewrite}[1]{{\textcolor{magenta}{\underline{#1}}}}
\newcommand{\outputsent}[1]{\textcolor{blue}{\{#1\}}}

\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{p{\linewidth}}
\hline
\multicolumn{1}{c}{(a) Zero-shot Prompt} \\
\textbf{\texttt{Here is some text:\inputsent{That is an ugly dress}. Rewrite it to be \rewrite{more positive}.}}
\\
\hline
\multicolumn{1}{c}{(b) Few-shot Prompt}\\
\texttt{Here is some text:\inputsent{I was really sad about the loss}. Rewrite it to be \rewrite{more positive}.}
\newline
\texttt{\outputsent{I was able to accept and work through the loss to move on.}}
\newline
\texttt{Here is some text:\inputsent{The eggnog was tasteless.}. Rewrite it to be \rewrite{more positive}.}
\newline
\texttt{\outputsent{The eggnog had a great, festive taste to it.}}
\newline
\texttt{`Here is some text:\inputsent{Everything is awful}. Rewrite it to be \rewrite{more positive}.}
\newline
\texttt{\outputsent{Everything is going well!}"}\newline
\textbf{\texttt{``Here is some text:\inputsent{That is an ugly dress}. Rewrite it to be \rewrite{more positive}.}}
\\
\hline
\multicolumn{1}{c}{(c) Augmented Zero-shot Prompt}
\\
\texttt{Here is some text:\inputsent{When the doctor asked Linda to take the medicine, he smiled and gave her a lollipop.}. Rewrite it to be \rewrite{more scary}. \newline
\outputsent{When the doctor told Linda to take the medicine, there had been a malicious gleam in her eye that Linda didn't like at all.} \newline
Here is some text:\inputsent{they asked loudly, over the sound of the train.}. Rewrite it to be \rewrite{more intense}. \newline
\outputsent{they yelled aggressively, over the clanging of the train}\newline
Here is some text:\inputsent{When Mohammed left the theatre, it was already dark out}.\newline
Rewrite it to be \rewrite{more about the movie itself}.\newline
\outputsent{The movie was longer than Mohammed had expected, and despite the excellent ratings he was a bit disappointed when he left the theatre.}\newline
Here is some text:\inputsent{next to the path}. Rewrite it \rewrite{to be about France}. \newline
\outputsent{next to la Seine}\newline
Here is some text:\inputsent{The man stood outside the grocery store, ringing the bell.}. Rewrite it to be \rewrite{about clowns}. \newline
\outputsent{The man stood outside the circus, holding a bunch of balloons.}\newline
Here is some text:\inputsent{the bell ringing}. Rewrite it to be \rewrite{more flowery}. \newline
\outputsent{the peals of the jangling bell}"\newline
Here is some text:\inputsent{against the tree}. Here is a rewrite of the text, which includes the word 'snow'. \newline
\outputsent{against the snow-covered bark of the tree}\newline
\textbf{\texttt{Here is some text:\inputsent{That is an ugly dress}. Rewrite it to be \rewrite{more positive}.}}}
\\
\hline
\end{tabular}
    \caption{Examples of zero, few and augmented-zero shot prompts for negative-to-positive style transfer on the sentence ``That is an ugly dress."
    % The prompt marked (b) is the exact one we used for all our style transfer experiments. The text corresponding to the specific example we would like to transform is marked in blue.
    }
    \label{tab:prompts}
\end{table*}

==> tables/selected_usage_examples.tex <==
\begin{table*}[ht]
\begin{adjustwidth}{-2cm}{}
    \small
    \centering
    \def\arraystretch{1.5}% 
    \begin{tabular}{p{0.41\linewidth} p{0.45\linewidth}}
    \toprule
      \textbf{Input} & \textbf{Model suggestion} \\ \hline
      I look around, noticing people from all ethnic backgrounds. I’m in shock, because my grandma was, well, a grandma. She liked cats and cooking for her family. She only had a flip phone. \newline \textbf{Rewrite it to be more descriptive.} & At first glance i noticed the difference in ethnicity, with people of all different skin tones. Then I remembered that my grandma was white as a ghost. She's never been to a concert, and has never touched an iPhone. \\ \hline
      You honor me," said Bruno. As he spoke, he began to laugh. His laugh was merry sounding and melodic. He took a deep breath. When he spoke again, his voice was low and strong. "I take this great task on and with my brothers shall lead us on to victory! \newline \textbf{Rewrite it to be about mining.} & You honor me, said Bruno. As he spoke, he began to laugh. His laugh was deep and gravely, as if from the bowels of the earth. He took a deep breath. When he spoke again, his voice was deep and dark. "I take this great task on and with my brothers shall delve into the mines!" \\ \hline
      I reckon,' smiled Toe, 'you'd have to say the same for icicles, wouldn't you? \newline \textbf{Rewrite it to be more interesting.} & ‘I reckon,’ smiled Toe, ‘you’d have to say the same for icicles, wouldn’t you?’ These words were barely out of his mouth before the others realized exactly what they meant.\\ \hline
      Anna Wintour, editor-in-chief of Vogue magazine, says it has tried to take steps to address some of the problems of fast fashion. \newline \textbf{Rewrite it to be more philosophical.} & Anna Wintour claims the solution to the fast fashion industry is the evolution of conscious consumers. \\ \hline
      But Sally remained unmoved--and lonely. \newline \textbf{Rewrite it to be more emotional} & Her tears rolled and rolled down her cheek, mixing with the saltwater around her, until the water was a rich mixture of the two. She wanted her poem to be cheerful like it used to be, but couldn't find the right words. \\
    \bottomrule
    \end{tabular}
    \caption{Examples of users' arbitrary style transfer requests for which the model suggestion was accepted.}
    \label{tab:selected_usage_examples}
    \end{adjustwidth}
\end{table*}

==> tables/yelp_comparison.tex <==

\begin{table*}
    \setlength{\tabcolsep}{2pt}
    \begin{subtable}{.58\linewidth}
    \centering \small 
        \begin{tabular}{l r r r}
        \toprule
         & Acc & BLEU & PPL\\
        \midrule
        Cross-alignment \citep{NIPS2017_2d2c8394} & 73.4 & 17.6 & 812 \\
        Backtrans \citep{prabhumoye-etal-2018-style} & 90.5 & 5.1 & 424 \\
        Multidecoder \citep{AAAI1817015}  & 50.3 & 27.7 & 1,703\\
        Delete-only \citep{li-etal-2018-delete} & 81.4 & 28.6 & 606 \\
        Delete-retrieve \citep{li-etal-2018-delete} & 86.2 & 31.1 & 948\\
        Unpaired RL \citep{xu-etal-2018-unpaired} & 52.2 & 37.2 & 2,750\\
        Dual RL \citep{DBLP:conf/ijcai/LuoLZYCSS19} & 85.9 & 55.1 & 982\\
        Style transformer \citep{dai-etal-2019-style} & 82.1 & 55.2 & 935\\
        \midrule
        % \underline{Augmented Zero-shot Prompting} \\
        GPT-3 ada, aug zero-shot& 31.5 & 39.0 & 283\\
        GPT-3 curie, aug zero-shot& 53.0 & 48.3 & 207\\
        GPT-3 da vinci, aug zero-shot& 74.1 & 43.8 & 231\\
        \midrule
        GLM, zero-shot \\ 
        GLM, five-shot \\
        GLM, aug zero-shot \\
        \midrule
        GLM-dialog, zero-shot \\
        GLM-dialog, five-shot \\
        GLM-dialog, aug zero-shot \\
        % \midrule
        % GLM & 65.0 & 49.3 & 292 & 10.3 \\
        % GLM-dialog & 73.7 & 40.6 & 184 & 10.7 \\
        % GLM & 79.6 & 16.1 & 173 \\
        % GLM-dialog & 90.6 & 10.4 & 79\\
        \bottomrule
        \end{tabular}
        \label{tab:prior-methods}
        \caption{}
    \end{subtable}
    \begin{subtable}{.40\linewidth}
    \centering \small 
        \begin{tabular}{l r r r}
        \toprule
         & Acc & BLEU & PPL\\
        \midrule
        \underline{GLM} \\
        Zero-shot & 69.7 & 28.6 & 397 \\
        + cand.~selection & 31.4 & 61.5 & 354\\
        Five-shot & 83.2 & 19.8 & 240\\
        + cand.~selection & 61.5 & 55.6 & 306\\
        Augmented zero-shot & 79.6 & 16.1 & 173\\
        + cand.~selection & 65.0 & 49.3 & 292\\
        \midrule
        \underline{GLM-dialog} \\
        Zero-shot & 59.1 & 17.6 & 138\\
        + cand.~selection & 46.8 & 24.2 & 166\\
        Five-shot & 94.3 & 13.6 & 126\\
        + cand.~selection & 81.3 & 47.6 & 345\\
        Augmented zero-shot & 90.6 & 10.4 & 79\\
        + cand.~selection & 73.7 & 40.6 & 184\\
        \bottomrule
        \end{tabular}
        \caption{}
        \label{tab:ablation}
    \end{subtable}
    % \vspace{3mm}
\caption{
For sentiment style transfer, we show accuracy, BLEU, and perplexity (PPL) reported as the average of positive $\rightarrow$ negative and negative $\rightarrow$ positive. 
In (a), augmented zero-shot prompting of GLM and GPT-3 are compared with prior supervised style transfer methods.
In (b), we compare zero-shot, five-shot, and augmented zero-shot prompting for our GLM models. 
Candidate selection means that of the sixteen examples returned by the API, we choose the one with the highest BLEU with the source sentence (in the default case, we just use the first returned output).  
}
\end{table*}
% \end{wraptable}

==> tables/yelp_comparisons_with_length.tex <==

% \begin{table}
%     \setlength{\tabcolsep}{2pt}
%     \centering \small 
%     \begin{tabular}{l r r r r}
%     \toprule
%      & Acc & BLEU & PPL & $l$\\
%     \midrule
%     Cross-alignment \citep{NIPS2017_2d2c8394} & 73.4 & 17.6 & 812 & 10.7 \\
%     Backtrans \citep{prabhumoye-etal-2018-style} & 90.5 & 5.1 & 424 & 9.7 \\
%     Multidecoder \citep{AAAI1817015}  & 50.3 & 27.7 & 1,703 & 10.4 \\
%     Delete-only \citep{li-etal-2018-delete} & 81.4 & 28.6 & 606 & 12.1 \\
%     Delete-retrieve \citep{li-etal-2018-delete} & 86.2 & 31.1 & 948 & 11.7 \\
%     Unpaired RL \citep{xu-etal-2018-unpaired} & 52.2 & 37.2 & 2,750 & 9.4 \\
%     Dual RL \citep{DBLP:conf/ijcai/LuoLZYCSS19} & 85.9 & 55.1 & 982 & 10.1 \\
%     Style transformer \citep{dai-etal-2019-style} & 82.1 & 55.2 & 935 & 10.3 \\
%     \midrule
%     \underline{Augmented Zero-Shot Prompting} \\
%     GPT-3 ada & 31.5 & 39.0 & 283 & 10.0 \\
%     GPT-3 curie  & 53.0 & 48.3 & 207 & 10.3 \\
%     GPT-3 da vinci  & 74.1 & 43.8 & 231 & 10.4 \\
%     \midrule
%     GLM & 65.0 & 49.3 & 292 & 10.3 \\
%     GLM-dialog & 73.7 & 40.6 & 184 & 10.7 \\
%     \bottomrule
%     \end{tabular}
%     \vspace{3mm}
%   \caption{
%           For sentiment style transfer, we show accuracy, BLEU, perplexity (PPL), and sequence length ($l$) for augmented zero-shot prompting compared with prior supervised style transfer methods.
%           Results shown are the average of positive $\rightarrow$ negative and negative $\rightarrow$ positive. 
%   \label{tab:prior-methods}
%   }
% \end{table}
% % \end{wraptable}



\begin{table}
    \setlength{\tabcolsep}{2pt}
    \begin{subtable}{.58\linewidth}
    \centering \small 
        \begin{tabular}{l r r r r}
        \toprule
         & Acc & BLEU & PPL & $l$\\
        \midrule
        Cross-alignment \citep{NIPS2017_2d2c8394} & 73.4 & 17.6 & 812 & 10.7 \\
        Backtrans \citep{prabhumoye-etal-2018-style} & 90.5 & 5.1 & 424 & 9.7 \\
        Multidecoder \citep{AAAI1817015}  & 50.3 & 27.7 & 1,703 & 10.4 \\
        Delete-only \citep{li-etal-2018-delete} & 81.4 & 28.6 & 606 & 12.1 \\
        Delete-retrieve \citep{li-etal-2018-delete} & 86.2 & 31.1 & 948 & 11.7 \\
        Unpaired RL \citep{xu-etal-2018-unpaired} & 52.2 & 37.2 & 2,750 & 9.4 \\
        Dual RL \citep{DBLP:conf/ijcai/LuoLZYCSS19} & 85.9 & 55.1 & 982 & 10.1 \\
        Style transformer \citep{dai-etal-2019-style} & 82.1 & 55.2 & 935 & 10.3 \\
        \midrule
        \underline{Augmented Zero-Shot Prompting} \\
        GPT-3 ada & 31.5 & 39.0 & 283 & 10.0 \\
        GPT-3 curie  & 53.0 & 48.3 & 207 & 10.3 \\
        GPT-3 da vinci  & 74.1 & 43.8 & 231 & 10.4 \\
        \midrule
        % GLM & 65.0 & 49.3 & 292 & 10.3 \\
        % GLM-dialog & 73.7 & 40.6 & 184 & 10.7 \\
        % GLM & 65.0 & 49.3 & 292 & 10.3 \\
        % GLM-dialog & 90.6 & 10.4 & 79 & 10.7 \\
        \bottomrule
        \end{tabular}
        \label{tab:prior-methods}
        \caption{}
    \end{subtable}
    \begin{subtable}{.40\linewidth}
    \centering \small 
        \begin{tabular}{l r r r r}
        \toprule
         & Acc & BLEU & PPL & $l$\\
        \midrule
        \underline{GLM} \\
        Zero-shot & 69.7 & 28.6 & 397 & 9.6 \\
        + cand.~selection & 31.4 & 61.5 & 354 & 10.2 \\
        Five-shot & 83.2 & 19.8 & 240 & 11.2 \\
        + cand.~selection & 61.5 & 55.6 & 306 & 10.2 \\
        Augmented zero-shot & 79.6 & 16.1 & 173 & 11.3 \\
        + cand.~selection & 65.0 & 49.3 & 292 & 10.3 \\
        \midrule
        \underline{GLM-dialog} \\
        Zero-shot & 59.1 & 17.6 & 138 & 17.2 \\
        + cand.~selection & 46.8 & 24.2 & 166 & 17.2  \\
        Five-shot & 94.3 & 13.6 & 126 & 13.3 \\
        + cand.~selection & 81.3 & 47.6 & 345 & 10.0 \\
        \textbf{Augmented zero-shot} & \textbf{90.6} & \textbf{10.4} & \textbf{79} & 12.8 \\
        + cand.~selection & 73.7 & 40.6 & 184 & 10.7 \\
        \bottomrule
        \end{tabular}
        \caption{}
        \label{tab:ablation}
    \end{subtable}
    \vspace{3mm}
\caption{
For sentiment style transfer, we show accuracy, BLEU, perplexity (PPL), and sequence length ($l$) reported as the average of positive $\rightarrow$ negative and negative $\rightarrow$ positive. 
In (a), augmented zero-shot prompting of GLM and GPT-3 are compared with prior supervised style transfer methods.
In (b), we compare zero-shot, five-shot, and augmented zero-shot prompting for our GLM models. 
Candidate selection means that of the sixteen examples returned by the API, we choose the one with the highest BLEU with the source sentence (in the default case, we just use the first returned output).  
}
\end{table}
% \end{wraptable}
